Ad-Rec: Advanced Feature Interactions to Address Covariate-Shifts in Recommendation Networks

Recommendation models are vital in delivering personalized user experiences by leveraging the correlation between multiple input features. However, deep learning-based recommendation models often face challenges due to evolving user behaviour and item features, leading to covariate shifts. Effective cross-feature learning is crucial to handle data distribution drift and adapting to changing user behaviour. Traditional feature interaction techniques have limitations in achieving optimal performance in this context. This work introduces Ad-Rec, an advanced network that leverages feature interaction techniques to address covariate shifts. This helps eliminate irrelevant interactions in recommendation tasks. Ad-Rec leverages masked transformers to enable the learning of higher-order cross-features while mitigating the impact of data distribution drift. Our approach improves model quality, accelerates convergence, and reduces training time, as measured by the Area Under Curve (AUC) metric. We demonstrate the scalability of Ad-Rec and its ability to achieve superior model quality through comprehensive ablation studies.

==> body/method.tex <==
\begin{figure*}[h]
	\centering
	\includegraphics[width=1\textwidth]{./body/Figures/Recomodel.pdf}
	\caption{\textbf{(a)} Non-sequential deep learning based recommendation model~\citep{dlrm}. They comprise of MLPs and embedding tables for processing dense and sparse inputs. Traditional dot product or concatenation-based feature interaction is deployed for finding similarities between input features. \textbf{(b)} \rectra: Recommendation model with transformer-based feature interaction for learning interaction between input features for improving model quality. Input features embedding feed the standard Transformer Encoder~\citep{attention} that performs feature interaction and learns the interactions.}
	\label{fig:model}
\end{figure*}

\section{Method}
\label{sec:method}

Figure~\ref{fig:model}\textbf{(a)} showcases the general model architecture of non-sequential deep learning-based recommendation models.
%
These models are currently one the largest ML workloads being deployed in datacenters~\citep{dsi}. 
%
They take two types of inputs namely dense and sparse.
%
Dense inputs comprise of continuous features like the user's age or time of the day while sparse inputs are categorical features such as the user's location or video being liked by the user.
%
Dense inputs are processed by neural networks like Multi-Layer Perceptrons (MLP).
%
Sparse inputs are handled by massive embedding tables of the order of 100s of Giga-Bytes (GBs).
%
Each embedding table represents a categorical feature with a number of rows representing possible items related to the feature.
%
As each user only interacts with a small fraction of these items in an embedding table, leaves the input vectors incredibly sparse resulting in random memory access.
%
Dense and sparse feature embeddings are passed through a dot product or concatenation-based interaction layer to find the similarities between the features.
%
Respective similarities are processed by another neural network to provide the final prediction (e.g., click-through rate) of how likely the user will interact with the recommendation.

\subsection{Transformer-based Feature Interaction (RecTra)}
\label{subsec:rectra}

\rectra~follows the original transformer~\citep{attention} to perform feature interaction as shown in Figure~\ref{fig:model}\textbf{(b)}.
%
Transformers have become the state-of-the-art method in many NLP tasks based on their efficient sequential learning.
%
A sequence of words is encoded as token embeddings and with added positional encoding is passed to the transformer encoder for learning the correlation of each word in the sequence.
%
For recommendation models, Bottom MLP $(\mathrm{MLP_{bot}})$ processes dense inputs $\mathbf{x_{dense}}$ into a single vector represented by $\mathbf{y_{dense}}$~(Eq.~\ref{eqn:1}).
%
Sparse inputs $\mathbf{x_{sparse}}$ (single-hot or multi-hot encoded) are processed by embedding lookup operation (with respective embedding table $\mathbf{E} \in \mathbb{R}^{M \times D}$) to generate a single embedding vector $\mathbf{y_{sparse}}$~(Eq.~\ref{eqn:2}).
%
$M$ defines the number of items in current feature embedding $\mathbf{E}$ and $D$ is the sparse feature size that is a hyper-parameter.
%
Output of dense and sparse features are concatenated~(Eq.~\ref{eqn:3},~\ref{eqn:4}) to generate feature sequence $\mathbf{z_{0}} \in \mathbb{R}^{1 \times (N+1)D}$.
%
This is equivalent to the 1D sequence of word token embeddings where the transformer uses constant latent vector size through all of its layers.
%
In the case of recommender systems, it represents the sequence of input feature embeddings where each feature comprises of constant latent vector size of $D$ as per the requirement of transformers.
%
Conventional DLRM either passes $\mathbf{z_{0}}$ directly or perform dot-product based feature interaction $lower\;trianlge(\;\mathbf{z_{0}} \times \mathbf{z_{0}^{T}}\;)$ to find correlation of input features.


\begin{flalign}
    \mathbf{y_{dense}} & = \mathrm{MLP_{bot}}\mathbf{(x_{dense})} &  \label{eqn:1} \\
    \mathbf{y_{sparse}} & = \mathbf{x_{sparse}}\mathbf{E} & \mathbf{E} \in \mathbb{R}^{M \times D}   \label{eqn:2}\\
    \mathbf{z_{0}} & = [\mathrm{MLP}(\mathbf{x_{dense}}) ; \mathbf{x_{sparse}^{1}}\mathbf{E^{1}} ; & \nonumber \\
    & \quad \quad \; . \; . \; . \; . \; ; \; \mathbf{x_{sparse}^{N}}\mathbf{E^{N}}\;] & \label{eqn:3} \\  
    %\mathbf{z_{0}} & = [\;\mathrm{MLP}(\mathbf{x_{dense}})\; ; \mathbf{x_{sparse}^{1}}\mathbf{E^{1}}\; ; \mathbf{x_{sparse}^{2}}\mathbf{E^{2}}\; ; . \; . \; . \; ; \; \mathbf{x_{sparse}^{N}}\mathbf{E^{N}}\;] & \label{eqn:3}\\
    \mathbf{z_{0}} & = [\;\mathbf{y_{dense}\; ; y_{sparse}^{1} \; ; & \nonumber \\
    & \quad \quad \; . \; . \; . \; . \; ; \; \mathbf{y_{sparse}^{N}}\;]} &   \label{eqn:4}\\
    %\mathbf{z_{0}} & = [\;\mathbf{y_{dense}\; ; y_{sparse}^{1}\; ; y_{sparse}^{2}\; ; . \; . \; . \; ; \; y_{sparse}^{N}\;]} &   \label{eqn:4}\\
    \mathbf{z^{'}_{\ell}} & = \mathrm{MSA}(\;\mathrm{LN}(\mathbf{z_{\ell - 1}})\;) + \mathbf{z_{\ell - 1}} & \ell = 1 . . . \mathb{L} \label{eqn:5}\\
    \mathbf{z_{\ell}} & = \mathrm{MLP}(\;\mathrm{LN}(\mathbf{z^{'}_{\ell}})\;) + \mathbf{z_{\ell}} & \ell = 1 . . . \mathb{L} \label{eqn:6}\\
    \mathbf{z_{\mathb{T}}} & = [\;\mathbf{y_{dense}}\; ; \mathbf{z_{\mathb{L}}}\;] &  \label{eqn:7}\\ 
    \mathrm{CTR} & = \mathrm{MLP_{top}}(\mathbf{z_{\mathb{T}}}) &  \label{eqn:8}
\end{flalign}

\if 0
%\vspace{-2ex}
\begin{flalign}\label{eqn:2}
    \mathbf{y_{sparse}} & = \mathbf{x_{sparse}}\mathbf{E} & & \quad
\end{flalign}

%\vspace{-2ex}
\begin{flalign}\label{eqn:3}
    \mathbf{z_{0}} & = [\;\mathrm{MLP}(\mathbf{x_{dense}})\; ; \mathbf{x_{sparse}^{1}}\mathbf{E^{1}}\; ; \mathbf{x_{sparse}^{1}}\mathbf{E^{2}}\; ; . \; . \; . \; ; \; \mathbf{x_{sparse}^{1}}\mathbf{E^{N}}\;] & \mathbf{E} \in \mathbb{R}^{m \times n} & \quad \quad
\end{flalign}

%\vspace{-2ex}
\begin{flalign}\label{eqn:4}
    \mathbf{z_{0}} & = [\;\mathbf{y_{dense}\; ; y_{sparse}^{1}\; ; y_{sparse}^{2}\; ; . \; . \; . \; ; \; y_{sparse}^{N}\;]} &  & \quad \quad
\end{flalign}

%\vspace{-2ex}
\begin{flalign}\label{eqn:5}
    \mathbf{z^{'}_{\ell}} & = \mathrm{MSA}(\;\mathrm{LN}(\mathbf{z_{\ell - 1}})\;) + \mathbf{z_{\ell - 1}} & \ell = 1 . . . \mathb{L} & \quad \quad
\end{flalign}

%\vspace{-2ex}
\begin{fleqn}[\parindent]
\begin{equation}
    \hspace{0.2in}
    \mathbf{z_{\ell}} = \mathrm{MLP}(\mathrm{LN}(\mathbf{z^{'}_{\ell - 1}})) + \mathbf{z_{\ell}} , \hspace{2.35in}  \ell = 1 . . . \mathb{L}
\end{equation}
\end{fleqn}\

%\vspace{-1ex}
\begin{fleqn}[\parindent]
\begin{equation}
    \hspace{0.2in}
    \mathrm{CTR} = \mathrm{MLP}(\mathbf{z_{\ell}})
\end{equation}
\end{fleqn}
\fi

\paragraph{Positional Embedding.}
For language tasks, position embeddings are added to the word embeddings to retain the positional information of a word in a sentence.
%
As the same word can appear at multiple positions across a sentence.
%
In the case of non-sequential recommender systems, position embedding is not required as neither the respective position of any feature changes in any input feature sequence nor the feature can appear in any other feature.
%
So the position of the feature does not encode any information that can be used to learn some information.
%
Concatenated input feature embeddings $\mathbf{z_{0}}$ serve as input to the encoder.
%
We have left the sensitivity study of using any sort of position embeddings - 1D position embedding and relative position embedding for future work. 

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{./body/Figures/seqrecmodel.pdf}}
\caption{High-level overview of sequential recommendation model. DLRM/RecTra acts as the base layer to generate a vector for a given user interaction event $\varepsilon$ at time $\tau$. Prior work~\citep{tbsm, gru4rec, attrec, transformers4rec} use multiple techniques to process time-based vectors of user sequential events.}
\label{fig:seqrecomodel}
\end{center}
\vskip -0.2in
\end{figure}

\paragraph{Transformer Encoder.}
The Transformer encoder consists of alternating layers of multi-headed self-attention (MSA, Appendix~\ref{subsec:MSA}) and MLP counterparts~(Eq.~\ref{eqn:5},\ref{eqn:6}).
%
Layernorm (LN) is applied either before or after every block and residual connections after every block~\citep{adaptive_input_repr_language, deep_translation_MT}.
%
Dropout can be controlled for residual connections.
%
The final output is passed through an MLP that can use either GELU or ReLU non-linearity.
%
The transformer encoder learns a deeper representation for each input feature by capturing the relation with each other input feature.
%
Query~($\mathbf{Q}$), Key~($\mathbf{K}$), and Value~($\mathbf{V}$) are extracted for each input feature through linear projection and fed to multi-head attention for finding relation of input features.
%
Non-linearity is being added using a feed-forward network and dropout to avoid overfitting.

The output of the last layer of the transformer is concatenated with processed dense inputs to generate $\mathbf{z_{\mathb{T}}}$~(Eq.~\ref{eqn:7}).
%
Top MLP $(\mathrm{MLP_{top}})$ processes $\mathbf{z_{\mathb{T}}}$ to provide the final click-through rate~(Eq.~\ref{eqn:8}).
%
To predict whether a user will click the target item, it is being modeled as a binary classification problem with binary cross-entropy loss~(Eq.~\ref{eqn:9}) where $y$ is the target and $p$ is the predicted probability.

\begin{equation}\label{eqn:9}    
    L = \sum{y\log(p) + (1 - y)\log(1 - p)}
\end{equation}


\subsection{Sequential Recommendation Models}
\label{subsec:seq_rec}

Sequential recommendation models explicitly incorporate timing components in terms of a set of events $\varepsilon$, where a user $u$ interacts with item $i$ and gave rating $r_{ui}$ at a particular time $t$. 
%
Single user interaction constitutes an event~$\varepsilon = \{ u, i, r_{ui}, t \}$.
%
User behavior can be represented in terms of a set of events for time $t = \{ 1, . . , \tau-1 \}$, and the job of the recommendation model is to predict the next event at time $\tau$.
%
Therefore, the training dataset $(S)$ is organized into a sequence of user activity, rather than simply a collection of user interaction with features in the case of non-sequential recommendation models.

Figure~\ref{fig:seqrecomodel} shows a high-level overview of sequential recommendation models where events $\varepsilon$ as input. 
%
To generate an embedding vector for each event, a standard DLRM model is used with an implicit timing component as a dense feature.
%
This generates a sequence of embedding vectors $Z$~(Eq.~\ref{eqn:10},\ref{eqn:11}).
%
Prediction of the next event relies on its context as well as its relevance to the earlier events~(Eq.~\ref{eqn:12}).
%
This relevance is being calculated in many ways by incorporating time series layer (TSL)~\citep{tbsm}, recurrent neural networks (RNN)~\citep{gru4rec}, multi-head attention (MHA)~\citep{attrec}, and even transformers~\citep{transformers4rec}.
%
This is passed through a final layer of MLP to generate the final probability of the next event $\varepsilon_{\tau}$.
%
As \rectra~works at the base of sequential recommendation models, so it can be used with any prior work to extract the relevance of events.
%
Embedding vector $\mathbf{z}_{t}$ generated by \rectra, represents the user-item interaction in a better way for the current event $\varepsilon_{t}$.
%
This implies that \rectra~ as the base model gives better results irrespective of the upper model.
%
%For current experiments, we show \rectra~improvement for sequential recommendation models with TSL as upper model.
%
%Improvement with other upper models are presented in Appendix.

\begin{flalign}
    \hspace{0.1in}
    \mathbf{z_{t}} & = \mathrm{DLRM/RecTra}\;(\varepsilon_{t}) & t = 1 . . . \tau \quad \quad \label{eqn:10} \\
    \hspace{0.1in}
    Z & = [\;\mathbf{z}_{1}, \mathbf{z}_{2}, . . , \mathbf{z}_{\tau-1}\;] & \quad \quad \label{eqn:11} \\
    \mathbf{c} & = \mathbf{attn}(\mathbf{z}_{\tau}, Z) & \quad \quad \label{eqn:12} 
\end{flalign}
\vspace{-0.28in}
\begin{equation}
    \min_{\theta} \sum_{(u,i) \in S} {(r_{ui} - \mathrm{MLP}(\mathbf{z}_{\tau}, \mathbf{c};\theta))}  \label{eqn:13}
\end{equation}

==> body/tables/new_seq_rec_models.tex <==
\begin{table}[h!]
\vspace{-0.05in}
\centering
\caption{Sequential Recommendation Model Architecture}
%\scriptsize
%\newcolumntype{?}{!{\vrule width 2pt}}
%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
%\setlength\extrarowheight{4pt}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{ c | c | c | c c | c c}
\hline
%
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Dataset}} & \textbf{Sequence} & \multicolumn{2}{c|}{\textbf{Features}} & \multicolumn{2}{c}{\textbf{Sequential Layer}} \\
\cline{4-7} & & \texbf{Length} & \textbf{Dense} & \textbf{Sparse} & \textbf{Type} & \textbf{Layers/Heads} \\
\hline
RM4 & \multirow{2}{*}{Taobao} & \multirow{4}{*}{21} & \multirow{4}{*}{1} & \multirow{4}{*}{3} & TSL & 1 \\
RM5 &  & & & & MHA & 8 \\
RM6 & \multirow{2}{*}{Alibaba} &  & & & RNN & 5 \\
RM7 &  &  & & & Transformer & 1 \\
 \hline
\end{tabular}}
\label{table:new_seq_rec_model}
\vspace{-0.1in}
\end{table}

==> body/tables/seq_metric.tex <==
\begin{table}[h!]
\centering
\caption{Evaluation Metric Comparison with single Epoch.}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{ l | c c | c c | c c}
\hline
%
\multirow{2}{*}{\textbf{Model}} &  \multicolumn{2}{c|}{\textbf{AUC}} & \multicolumn{2}{c|}{\textbf{Test Accuracy (\%)}} & \multicolumn{2}{c}{\textbf{BCE Loss}}
\\
 & \textbf{TBSM} & \textbf{\rectra} & \textbf{TBSM} & \textbf{\rectra} & \textbf{TBSM} & \textbf{\rectra} 
\\
\hline
RM4 (TSL) & 0.928  & \textbf{0.949}  & 89.25 & \textbf{90.78} & 0.265 & \textbf{0.231}  \\
RM5 (MHA) & 0.866  & \textbf{0.892}  & 82.80 & \textbf{84.31} & 0.386 & \textbf{0.361}\\
RM6 (RNN) & 0.844  & \textbf{0.847}  & \textbf{83.62} & 81.95 & \textbf{0.381} & 0.410  \\
RM7 (Transformer) & 0.924  & \textbf{0.931}  & 88.19 & \textbf{88.57} & 0.288 & \textbf{0.280}  \\
 \hline
\end{tabular}}
\label{table:seq_metric}
\end{table}

==> body/tables/seq_models.tex <==
\resizebox{1\textwidth}{!}{
\begin{tabular}{c | l | c | c c | c c c | c c | c c c c | c c}
\hline
%
\multirow{4}{*}{\textbf{Model}} & \multirow{4}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Sequence}} & \multicolumn{11}{c|}{\textbf{Non-Sequential Recommendation Model: DLRM / \rectra}} & \multicolumn{2}{c}{\textbf{Sequential Layer}} \\
\cline{4-16} & & & \multicolumn{2}{c|}{\textbf{Features}} & \multicolumn{3}{c|}{\textbf{Parameters}} &  \multicolumn{2}{c|}{\textbf{MLP Config}} & \multicolumn{4}{c|}{\textbf{Transformer Encoder Configuration}} & \multirow{3}{*}{\textbf{Type}} & \textbf{Layers}
\\
\cline{4-14} &  & \multirow{2}{*}{\textbf{Length}} & \multirow{2}{*}{\textbf{Dense}} & \multirow{2}{*}{\textbf{Sparse}} & \multirow{2}{*}{\textbf{Dense}} & \multirow{2}{*}{\textbf{Sparse}} & \textbf{Sparse} & \multirow{2}{*}{\textbf{Bot}} & \multirow{2}{*}{\textbf{Top}} & \textbf{Num} & \textbf{Num} & \textbf{Hidden} & \textbf{Linear} & & \textbf{/} \\
 & &  & & & & & \textbf{Dim} & & & \textbf{Layers} & \textbf{Heads} & \textbf{Size} & \textbf{Config.} & & \textbf{Heads} \\
\hline
RM4 & Taobao & \multirow{3}{*}{21} & 1 & 3 & 7.3k & 5.1M & 16 & 1-16 & 15-15 & 1 & 2 & 16 & 512 & TSL & 1 \\
RM5 & \multirow{2}{*}{Alibaba} &  & 1 & 3 & 7.3k & 5.1M & 16 & 1-16 & 15-15 & 1 & 2 & 16 & 512 & MHA & 8 \\
RM6 &  &  & 1 & 3 & 7.3k & 5.1M & 16 & 1-16 & 15-15 & 1 & 2 & 16 & 512 & LSTM & 5 \\
 \hline
\end{tabular}}
